ALDi: Quantifying the Arabic Level of Dialectness of Text

Transcribed speech and user-generated text in Arabic typically contain a mixture of Modern Standard Arabic (MSA), the standardized language taught in schools, and Dialectal Arabic (DA), used in daily communications. To handle this variation, previous work in Arabic NLP has focused on Dialect Identification (DI) on the sentence or the token level. However, DI treats the task as binary, whereas we argue that Arabic speakers perceive a spectrum of dialectness, which we operationalize at the sentence level as the Arabic Level of Dialectness (ALDi), a continuous linguistic variable. We introduce the AOC-ALDi dataset (derived from the AOC dataset), containing 127,835 sentences (17% from news articles and 83% from user comments on those articles) which are manually labeled with their level of dialectness. We provide a detailed analysis of AOC-ALDi and show that a model trained on it can effectively identify levels of dialectness on a range of other corpora (including dialects and genres not included in AOC-ALDi), providing a more nuanced picture than traditional DI systems. Through case studies, we illustrate how ALDi can reveal Arabic speakers' stylistic choices in different situations, a useful property for sociolinguistic analyses.

==> abandoned-ideas.tex <==
\section{Introduction}
% IDEA - Language Identification (LI) is achieved for distant languages
Automatic Language Identification (LI) is the task of determining the natural language for a piece of text. Features such as ngram counts and language model perplexity showed to be effective for discriminating between distant languages that have low lexical overlap or even use completely different scripts \cite{jauhiainen2019automatic}.
%IDEA - Language Identification of a piece of text is not solved for similar languages.
%The problem is even harder for dialects of the same language.
However, the task is far from being solved for similar languages such as South Slavic languages - namely Bosnian, Croatian, and Serbian - and for dialects of the same language as in English (e.g, British English and American English), Portuguese (e.g, Brazilian Portuguese and European Portuguese), and Arabic (e.g., Modern Standard Arabic and Egyptian Arabic). The differences between these variants are more subtle than between distant languages causing the task to be challenging. For written text, some of the phonological features that are distinctive of these dialects are lost making distinguishing between them even harder. \todo{Add references}

%IDEA - People generally look for distinctive markers of the dialects to distinguish between them.
Humans generally look for remaining distinctive markers of these similar variants (dialects or similar languages) as cues to perform dialect identification. For some sentences, overt cues are available, but for others, the cues are really nuanced or even missing. 
%IDEA - Dialect identification assumes the markers to be of the same, in the sense that the appearance of any of them is enough to consider the whole sentence to be written in a specific dialect.
The task of Dialect Identification assumes that the distinctive markers are of the same importance for determining the dialect of a sentence. More specifically, the appearance of any subtle dialectal feature is enough to consider the whole sentence to be written in the dialect relevant to this feature. This definition neglects the differences between different dialectal sentences and terms.
%IDEA - This is problematic as some markers are signs of dialectness, yet are not distinctive of a specific dialect.
Moreover, sentences are generally assigned to a specific variant which is not suitable for ones that are clearly dialectal yet can be assigned to different dialects as the cues found within the sentences are used in different dialects.

\textarabic{تفائلوا شوي} (Gulf and Levantine)

\textarabic{ياخي شوي شوي لاتطير في العجه} (Gulf) \todo{\url{https://www.alriyadh.com/1684566}}

\textarabic{و هاد شي اسمو شحده بس ستايل شوي} (Levantine)

\todo[inline]{ALDi affects intelligibility? }
%IDEA - The main contributions are
%IDEA Proposing to use level of dialectness as a continuous spectrum, instead of having a single dialect label for the sentence.
%IDEA Providing baselines and a supervised model for estimating the level of dialectness of a sentence
%IDEA This metric can be used to enrich sociolinguistic analysis by studying how the level of dialectness differs according to different factors.
%IDEA Analyzing the level of dialectness of sentences of specific corpora (Lyrics of Arabic songs?, Subtitles of Arabic movies, Speeches of political Arabic figures?)
Therefore, we define a new task meant to estimate the \textit{Arabic Level of Dialectness} (ALDi) of a sentence. Instead of classifying a sentence as either dialectal or not, we propose to have a continuous spectrum for the dialectness of the sentence. The main contributions of our paper can be summarized as follows:
\begin{enumerate}
    \item Motivating the \textit{Arabic Level of Dialectness} (ALDi) as a new linguistic variable that distinguishes between different dialectal sentences, and presenting it as a new task for the Natural Language Processing (NLP) community.
    \item Re-releasing Arabic sentences with their ALDi labels from the Arabic Online Commentary (AOC) dataset \cite{zaidan-callison-burch-2011-arabic}, and providing canonical splits of these samples.
    \item Using supervised and unsupervised models for automatically estimating the ALDi of Arabic sentences.
    \item Demonstrating how the ALDi variable provides a quantitative metric that can enrich sociolinguistic studies. We perform a quantitative replication for a qualitative study that analyzed how two former Arab presidents used their dialects in their speeches \cite{lahlali2011arab}. The results showcase the capability of the metric to replicate studies that could previously only be performed qualitatively.
\end{enumerate}


\section{Background}
%IDEA - Languages vs dialects (salient differences to subtle ones)
Human languages are experiencing continuous evolution, and change. These evolution processes are further stimulated by the interaction between people speaking different languages, which causes them to impact each other, and might result in making these languages diverge from other languages belonging to the same family. The case also holds for dialects of the same language which tend to be affected by each other, and by contact with other local languages.
\todo{TODO: Better understand the difference between “vernacular”, “colloquial”, “slang”, and “dialectal”.}

%IDEA - Defining Standard English is complicated
%IDEA - RP (Received Pronunciation) is not enough
%IDEA - The presence of Standard American English, Standard British English, … shows it is not a single language.
%IDEA - It can be assumed to be a dialect of English (Trudgill,  )
We hypothesize there are two categories of languages based on what the language speakers perceive to belong to the standard language as opposed to belonging to a dialect of the language. The first category of languages applies to English, in which multiple standard forms of the language are present (e.g., Standard American English, Standard British English, Standard Australian English), in addition to multiple dialects and vernaculars such as African American Vernacular English (AAVE). Defining what a standard variant of the language is not straightforward. While Received Pronunciation (RP) is traditionally perceived as the standard British accent, \citet{trudgill2002standard} argued that Standard English can itself be defined as another dialect of English that is the most popular one and is widely taught in schools.
%IDEA - For Arabic and German, there seems to be an agreed-upon (to some extent) Standard language that is used in written newspapers, in addition to various dialects.
%IDEA - In this case, Level of Dialectness of a piece of text might be a great indicator of the Formality of the text.
On the other hand, the second category encompasses languages such as Arabic, and German in which the standard language can be agreed upon to some extent. The standard language in this case has standardized orthography, and grammar that are taught in schools, and strictly followed in written text such as newspapers. Conversely, dialects of these languages are mostly spoken and have no standardized written form. With the rise of social media platforms, speakers of these different dialects are sharing their thoughts online using their native dialects, mostly writing dialectal words using spellings that would match how they pronounce them. \todo{Where does Portuguese lie in this categorization?} \todo{Clarify that German might be similar but we are not sure and it needs more investigation.}

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.5\textwidth]{images/dialectness-and-formality.pdf}
    \caption{Intuition on the relationship between the level of dialectness and the formality of text.}
    \label{fig:level-of-dialectness-vs-formality}
\end{figure}

\subsection{The Dialect Identification task}
\label{sec:di}
% IDEA - Defining Dialect Identification
Dialect Identification is the task of predicting the dialect in which a piece of text is written. It can be viewed as an extension of the language identification task.
% IDEA - How the task is operationalized?
% IDEA - Detecting the dialectal features
Different approaches were deployed to define the dialect identification task. \citet{demszky-etal-2021-learning} identified 22 distinctive features of Indian English and compared the ability of regular expressions, and fine-tuned BERT models in detecting these features.
% IDEA - DI as sentence classification
On the other hand, multiple papers attempt to consider dialect identification as a sentence classification task in which a model predicts the most probable dialect for a piece of text out of a predefined set of dialects (\citealt{zaidan-callison-burch-2011-arabic}; \citealt{lui-cook-2013-classifying}; \citealt{maier-gomez-rodriguez-2014-language}; \citealt{zampieri-etal-2014-report}; \citealt{sadat-etal-2014-automatic}; \citealt{darwish-etal-2014-verifiably}; \citealt{mubarak-darwish-2014-using}; \citealt{salama-etal-2014-youdacc}; \citealt{alshutayri2017exploring}; \citealt{alsarsour-etal-2018-dart}; \citealt{zaghouani-charfi-2018-arap}; \citealt{charfi-etal-2019-fine}; \citealt{bouamor-etal-2019-madar}; \citealt{el-haj-2020-habibi}; \citealt{9310507}; \citealt{abdul-mageed-etal-2020-nadi}; \citealt{abdul-mageed-etal-2021-nadi}; \citealt{abdelali-etal-2021-qadi}; \citealt{abdul-mageed-etal-2022-nadi}; \citealt{althobaiti_2022}; \citealt{zampieri2023language}). 
\todo[inline]{Describe the papers mentioned above!}

% IDEA - Dialect Identification for English includes a set of country-level labels

% IDEA - Dialect Identification for Arabic includes Standard Language as well

% IDEA - Dialect Identification for Swiss German
\todo[inline]{Dialects of Swiss German in VarDial}

\subsection{Relation between ALDi and Formality}
%IDEA - Formality of English is theorized to be related to Fuzziness (use of fuzzy and vague terms), and Context-Dependence (Heylighen and Dewaele,  )
Formality of a sentence can depend on the Fuzziness of the sentence (i.e.: how vague and unspecific some terms are), and the Context-Dependence of the sentence (i.e.: to what extent does the sentence rely on common knowledge shared by the interlocutors that can not be easily inferred without knowing the context in which the sentence is used) \cite{heylighen1999formality}.
%IDEA - Later papers refer to the usage of slang words and the presence of grammatical inaccuracies as signs of informal text.
Later operationalizations of formality refer to the impact factors such as slang words and grammatical inaccuracies impact people's perception of formality (\citealp{mosquera2012qualitative}; \citealp{peterson-etal-2011-email}) as cited in \cite{pavlick-tetreault-2016-empirical}.

%IDEA - For German and Arabic, level of dialectness is one metric that affects the formality of a sentence
For languages having a single variant of standard language, we hypothesize that the ALDi of a sentence is an indicator for the formality of the sentence as demonstrated in Figure \ref{fig:level-of-dialectness-vs-formality}. 
%IDEA - For languages of a standard variant that is used in formal written communications, we think “Level of Dialectness” is another dimension to differentiate between formal and informal text.
We argue that a sentence with a high ALDi is more likely to be informal. Dialects generally rely on context-dependent knowledge shared by the speakers of these dialects that might not be known to speakers of other dialects. Moreover, the spontaneous non-standardized writing system used for dialects might be perceived by some people to be violating the grammatical rule and the standardized orthography, which in turn would make them see the sentence as informal. Therefore, the ALDi can be seen as a combination of the fuzziness and the content-dependence features of a sentence that  \citet{heylighen1999formality} used to model the formality of sentences. Moreover, slang words are initially introduced to dialects before being integrated into the standard variants of languages. Therefore, using slang words that are known to be less formal is mainly linked to the usage of a dialect, thus motivating the relationship between the ALDi and the formality of text.
% IDEA - Annotating the level of dialectness is easier than annotating the formality of a piece of text, as multiple factors context can impact the formality.
We believe that estimating the level of dialectness of a sentence is less ambiguous than estimating its formality and hence propose it as a new NLP task in the subsequent section.


\section{The Arabic Level of Dialectness (ALDi) Task}
\label{sec:ALDi_task}
% IDEA - Definition: Level of dialectness of text refers to the extent to which the sentence diverges from the standard language by having signs of dialectness.
\todo[inline]{Have a more explicit definition?}
The \textit{Level of Dialectness} of a sentence refers to the extent by which the sentence diverges from the standard language. The divergence is mainly caused by the presence of distinctive markers of dialects that differ from the standard language. Some of these markers that are apparent in spoken utterances are lost in spoken text.
% IDEA  - Level of Dialectness is not new yet abandoned
As discussed in \S\ref{sec:di}, previous research mainly focused on assigning text to different dialects. This formulation ignores the fact that some sentences could be more dialectal than others. For Arabic, ALDi of a sentence is not formalized as an NLP task on the sentence level. However, multiple papers discuss the presence of a difference in the dialectness among Arabic sentences.

% IDEA - (Parkinson, 1991) sampled sentences from an editorial column
% IDEA - The annotators behaviour for detecting dialectal segments in sentences was interesting
\citet{10.2307/43192652} sampled sentences from an editorial column from an Egyptian newspaper (Al-Ahram) written by a journalist who is known to code-switch between dialectal Egyptian Arabic, and Modern Standard Arabic (MSA) in his writings. Ten subjects in addition to two linguistically trained native speakers were then asked to identify the dialectal segments within the sentences. The author noticed that people's ability to pronounce the whole sentence as being MSA or Egyptian Arabic affects the segments that they highlight as dialectal. The default position seems to consider that the sentence is written in MSA. On the appearance of a dialectal feature, the annotators would reevaluate the whole sentence which might result in them marking the whole sentence as dialectal.
% IDEA - They used three levels (MSA - Mixed - Dialectal) to classify sentences extracted from a column of a newspaper.
\todo[inline]{IDEA - They used three levels (MSA - Mixed - Dialectal) to classify sentences extracted from a column of a newspaper.}

% IDEA - (Zaidan and Callison-Burch, 2011) asked annotators to tag comments to online news articles for their dialect (Egyptian, Levantine, Gulf, Maghrebi, Iraqi, General, MSA), and their level of dialectness (Little, Mixed, Mostly, MSA).
\citet{zaidan-callison-burch-2011-arabic} shared the same intuition that sentences can be classified into multiple levels of dialctness namely MSA, little-dialectal, mixed, or mostly dialectal. They extracted comments to news articles from three different newspapers published in Egypt, Jordan, and Saudi Arabia. The comments were later evaluated by three human annotators for their dialect (Egyptian, Levantine, Gulf, Maghrebi, Iraqi, General, MSA) and their level of dialectness, forming the Arabic Online Commentary (AOC) dataset.
% IDEA - Annotators over-identify sentences as written in their native dialects
For the dialect label, the authors found that annotators tend to over-identify their own dialects (i.e., consider comments to be written in their own dialect even if the comment is accepted in other dialects) \cite{zaidan-callison-burch-2014-arabic}.
% IDEA - once again this might be related to the relation between perception of dialectness and pronunciation
This finding might be attributed to the fact that humans consider the text to be written in their native dialect if they can pronounce it in their dialect or in MSA. Therefore, there seems to be a strong relationship between people's perception of dialectness and their ability to pronounce sentences in their native dialects.
% IDEA - The authors and future papers using AOC ignored level of dialectness
\citet{zaidan-callison-burch-2014-arabic} focused on only analyzing the dialect label for each comment and ignored the annotations for the level of dialectness. Surprisingly, all subsequent papers that used the AOC dataset did the same. We speculate that researchers either did not that the comments are annotated for their level of dialectness or overlooked the importance of the Level of Dialectness of the comments. Moreover, the format of the original dataset is not user-friendly which might have also hindered the investigation of the ALDi label.


% IDEA - Previous relevant research
% IDEA - (Habash et al., 2008) proposed tagging each token as dialectal or MSA.
% IDEA - (Elfardy and Diab, 2012) simplified the token tagging scheme
From a modeling point of view, few attempts were done to quantify the ALDi but mainly on the token level.\todo{refer to code-switching papers as well? Lince?} \citet{habash2008guidelines} proposed a tagging scheme of 5 levels for determining the level of dialectness of each token within a sentence. Hand-crafted guidelines are then used to assign a 5-level segment dialectness annotation based on the distribution of the token tags within the segment. For a subset of 11 documents, annotators achieved lower agreement scores for the segment-level labels compared to the token-level ones. \citet{elfardy-diab-2012-simplified} took inspiration from \cite{habash2008guidelines} and created simplified and coarse-grained token-level annotation guidelines. Instead of determining the level of dialectness of a token on an ordinal 5-level scale, they determined 7 classes of tokens namely: (1) MSA, (2) DA, (3) Both MSA and DA, (4) Foreign words, (5) Named entities, (6) Typos, and (7) Unknown words. Human annotations of forum posts show that determining whether a term belongs to a variant of DA or to both MSA and DA is challenging and subjective. \todo{Mention the Algerian Arabic LI paper \cite{adouane-dobnik-2017-identification}}
% IDEA - (Sajjad et al., 2020) computed the percentage of tokens within a sentence not found in an MSA lexicon as a measure for the level of dialectness of different dialectal corpora.
Later on, \citet{sajjad-etal-2020-arabench} computed the percentage of tokens within a sentence not found in a lexicon of MSA tokens extracted from multiple sources as a proxy for the sentence-level dialectness, and used it to quantify the dialectness of different Arabic corpora.

% Abandoned IDEA - Moreover, \citet{elfardy-diab-2013-sentence} used the token-level dialect identification in order to perform sentence-level Dialect Classification between MSA and Egyptian Arabic \todo{on which dataset}.

\todo[inline]{\cite{Elfardy2017PerspectiveII} mentions MSA == Formal, DA == Informal}


==> old_introduction_background.tex <==
\section{Introduction}
% IDEA - Language Identification (LI)
Automatic Language Identification (LI) is the task of determining the natural language for a piece of text. Features such as ngram counts and language model perplexity showed to be effective for discriminating between distant languages that have low lexical overlap or even use completely different scripts \cite{jauhiainen2019automatic}.
% IDEA - Dialect Identification
That being said, LI systems' performance tends to degrade for closely related languages such as South Slavic languages - namely Bosnian, Croatian, and Serbian - or for variants (dialects) of the same language as in English (e.g, British English and American English), Portuguese (e.g, Brazilian Portuguese and European Portuguese), and Arabic (e.g., Modern Standard Arabic and Egyptian Arabic). Phonological differences between these variants are generally lost for written text. Thereafter, only the distinctive lexical, morphological, and syntactic features of these dialects showing in the written form can be used to achieve this fine-grained classification between them. 

% IDEA - Issue of defining standard language
The task of fine-grained variant identification is exacerbated by the need to distinguish between the standard variant of a language and the other dialects. \citet{trudgill2002standard} argued that Standard English is a set of dialects of English that is generally taught in schools, and widely used in newspapers and specific social situations which makes it the most important dialect of English. \todo{Improve the argument here}


The difference between the standard form of a language and its dialect is more salient in Arabic. The Arab countries share a situation called diglossia in which two forms of the language co-exist \citep{ferguson1959diglossia}. A high variant known as Modern Standard Arabic (MSA) is the official language of all the Arab countries and is perceived to be more prestigious and grammatically sound, taught in schools, yet is mostly written. On the other hand, lower sets of variants (dialects) exist that are widely spoken in everyday communications. While people rely on signals of dialectness in written and spoken forms to distinguish between MSA and Arabic dialects, \citet{10.2307/43192652} showed that they tend to disagree when the text has a mixture of both MSA and dialectal segments in the text. 

% IDEA - Introduce the problem
Instead of considering dialects as monolithic separate classes, we define \textit{level of dialectness} as a continuous spectrum that reflects how the appearance of dialectal features in a piece of text impacts the people's perception of this text. This would allow for better distinguishing between the different levels of dialectness within dialectal texts, by separating the highly dialectal texts from the free of dialectal features ones. 
% IDEA - Focus on Arabic dialects
While Arabic dialects are the main focus of the paper, we believe that the idea of the level of dialctness can be extended to other languages that have similar variants.

% IDEA - Applications
\todo[inline]{Application \#1: Enrich the analysis of dialectal text usage}
\todo[inline]{Application \#2: Use it as a metric for evaluating generation models that try to increase the Dialectness of the text}


\begin{table*}[htbp]
    \centering
    \begin{tabular}{lc}
        \textbf{Dialect} & \textbf{Sentence}\\
        \midrule
        American English &  I bought the \textbf{fries} from the market.\\
        British English & I bought the \textbf{chips} from the market.\\
        \midrule
        Egyptian Arabic & \textarabic{اشتريت \textbf{الأوطة} من السوق} \\
        Modern Standard Arabic (undiactrized) & \textarabic{اشتريت \textbf{الطماطم} من السوق} \\
        Modern Standard Arabic (diactrized) & \textarabic{ُاشتريت \textbf{َالطماطم} ِمنَ السوق} \\
        English Gloss & I bought the \textbf{tomatoes} from the market.\\
        \bottomrule
    \end{tabular}
    \caption{Examples of distinctive lexical terms between dialects}
    \label{tab:examples_distinctive_terms}
\end{table*}
\todo{Fix the diactrized example in the Table!}


\section{Background}
% IDEA - Language change is a feature of human languages 
Human languages have the unique feature of continuous evolution and change. Various factors cause this change from factors related to the continuous interaction between speakers of multiple languages, to sociolinguistic factors that might influence the change. 
% IDEA - Evolution might make variants of the same language to diverge
The continuous evolution might cause the variants of the same language to diverge from each other. Considering these variants to be dialects of the same language or separate languages is not clear cut. Language represents a part of a human's identity, and thus considering a variant of a language as a dialect or a separate language entails social and political factors that shape peoples' identities, and how they express themselves.

\todo[inline]{Get this section generic transitioning from Languages to Arabic}.

% IDEA - explain the state of Arabic, and why lots of variants exist.
Arabic is a Semitic language that has origins dating back to the \todo{Exact number} century. The language was generally spoken in the Arabian peninsula. It is also the language of the holy book of Islam (the Quran). With the spread of Islam across the Levantine and the North African countries, Arabic started to also spread as the language people speak, in addition to their own native languages. These countries also had been influenced by other neighbouring languages such as Turkish, and Persian, in addition to English, and French due to colonization.  All these factors caused Arabic as a language to exist in a state of diglossia, in which two languages exist side by side in each Arabic-speaking country. A higher standardized variant of the language, that has its grammar rules, resembles Classical Arabic (CA) that dates back to the 7th century. This variant is known to non-Arabic speakers and across the linguistics field as Modern Standard Arabic (MSA), to distinguish it from the CA. For most of the Arabic speakers, the term "Fus-ha" refers to both MSA and CA. That being said, "Fus-ha" is taught in schools, and generally used in newspapers, and . Moreover, lower variants of Arabic exists within each community, that are generally the languages people speak, and are referred to as "Amiya" or "Darija". These variants are considered as dialects of the Arabic language. The fact that Arabic is spoken across a widespread region, causes these dialects to be quite divergent from each other, to the extent that some dialects are not intelligible to speakers of other dialects. The differences between Arabic dialects within themselves and with MSA might be phonological, morphological, semantic, and syntactic. This makes Arabic a unique language for the study of dialectology, and language variation.

% IDEA - 


\todo[inline]{Main points}
\begin{itemize}
    \item Arabic DI as a task
    \begin{itemize}
        \item AOC (2011 and 2014)
        \begin{itemize}
            \item Elfardy (2013)
            \item Mageed (2018)
            \item Mo Elhaj (2018)
        \end{itemize}
        \item MADAR
        \item QADI
        \item NADI and its subtasks
    \end{itemize}
    \item Basic Level of Dialectness
    \begin{itemize}
        \item Nizar Habash (2008) and Elfardy (2012)
        \item Languages of Algeria paper (2017)
        \item Hassan Sajjad - Arabench (2020)
    \end{itemize}
    \item Fusha paper
    \item Dialectness in AOC
    \item Formality of English (Pevlick, ??)
    \begin{itemize}
        \item Slang is a bigger problem in Arabic since the MSA isn't really being revised and updated. Moreover, MSA isn't the same across different countries.
    \end{itemize}
    \item Level of Dialectness of Text is less than that of Speech (as pronunciation signals are dropped).
\end{itemize}

\todo[inline]{Extra valid points?}
\begin{itemize}
    \item AAVE
    \item Features of Indian English (NAACL 2021)
    \item Standard English paper
\end{itemize}


\begin{itemize}
    \item Define Level of Dialectness: In case of a clear Dialectal term: 100 - Percentage of words that can not have Dialectal pronunciations.
    \begin{itemize}
        \item Use Searching for fusha paper (1991) - how failure to pronounce word as MSA makes it DA. Is it the case that people first try to read it as MSA and when it fails give it a complete re-read as DA?
        \begin{itemize}
            \item Presence of a single Dialectal word would make people perceive text as dialectal.
            \item Presence of a fusha feature is not enough to make them flag the sentence as MSA.
        \end{itemize}
        \item In one of Eric Atwell's papers (2018 or 2019) they mention the number of MSA words
        \item Similarly, Nizar (2008) and Elfardy (2012) have a similar instantiation.
        \item Hassan Sajjad (2018? AraBench?) uses the percentage of tokens not in an MSA lexicon. 
    \end{itemize}
\end{itemize}

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.5\textwidth]{images/dialectness-and-formality.pdf}
    \caption{Intuition on the relationship between the level of dialectness and the formality of text.}
    \label{fig:level-of-dialectness-vs-formality}
\end{figure}

 
